Evaluating the word-expert approach for Named-Entity Disambiguation

Named Entity Disambiguation (NED) is the task of linking a named-entity mention to an instance in a knowledge-base, typically Wikipedia. This task is closely related to word-sense disambiguation (WSD), where the supervised word-expert approach has prevailed. In this work we present the results of the word-expert approach to NED, where one classifier is built for each target entity mention string. The resources necessary to build the system, a dictionary and a set of training instances, have been automatically derived from Wikipedia. We provide empirical evidence of the value of this approach, as well as a study of the differences between WSD and NED, including ambiguity and synonymy statistics.

==> heuristic.tex <==
\section{A Context-Sensitive Heuristic for Entity Disambiguation}
\label{sec:cont-sens-heur}

{\bf COPIED VERBATIM FROM TAC-KBP 2010 PAPER}

Our main context-dependent approach attempts to disambiguate an entity
mention by identifying other possible mentions of the same entity
in text.  The intuition here is that
while some acronyms (such as ``ABC'') are
ambiguous, there may be other mentions of the same entity in the
document that uniquely identify it (e.g., ``American Broadcasting Company'').
To keep things simple, we assume that the longest entity mention is
least ambiguous and use {\em{that}} in our dictionary lookup,
instead of the original mention.

We find the set of other possible mentions for a given entity's string
by first running the Stanford NER system~\citep{finkel-grenager-manning:2005:ACL}
on the document's text to find all entity names.
For all occurrences of the target entity string,
we determine whether it was part of a longer NER chunk.
We then use the Stanford deterministic
coreference system~\citep{raghunathan2010}
to find all entity names that are coreferent
with the target entity.
In addition, since our dictionary provides a list of
Wikipedia articles to which the target mention could refer,
we can identify all strings in the document matching any
of their titles.
We then use the longest string obtained by extending the
current entity mention to an NER chunk, coreference resolution,
and matching Wikipedia titles in the document, and use {\em{that}}
as the new entity name to query the dictionary.  This yields a
new set of possible matching Wikipedia articles.  To avoid noise
(say, from a bad coreference suggestion), we restrict this set,
intersecting it with the original list of possible Wikipedia titles,
obtained earlier (by using the original mention to query the
dictionary for possible articles).  Finally, we select the top-ranked
title from this set.

Below we give motivating examples for our proposed heuristics,
taken from the 2009 TAC-KBP entity linking evaluation:

{\footnotesize
\begin{center}\begin{tabular}{rp{15cm}}
String & {\tt{Abbott}} \mbox{ }\mbox{ }\mbox{ } [60 choices in the LNRM dictionary]\\
Top Choice & {\tt{Abbott\_Laboratories}} \\
Correct Choice & {\tt{Bud\_Abbott}} \\
Context & {\tt{Comedian Bud Abbott of Abbott and Costello died in Woodland Hills, California.}} \\
Heuristic & Expanding the target string, {\tt{Abbott}}, to the named entity span containing it,
{\tt{Bud Abbott}}, leads us to the correct entity.
\\\\
String & {\tt{ABC}} \mbox{ }\mbox{ }\mbox{ } [253 choices]\\
Top Choice & {\tt{American\_Broadcasting\_Company}} \\
Correct Choice & {\tt{All\_Basotho\_Convention}} \\
Context & {\tt{$\ldots$say victory over the newly-formed All Basotho Convention ( ABC ) is far from certain$\ldots$}} \\ 
Heuristic & Using coreference resolution to match the target string, {\tt{ABC}}, to {\tt{All Basotho Convention}}, correctly determines the entity.
\\\\
String & {\tt{ABC}} \mbox{ }\mbox{ }\mbox{ } [still 253 choices]\\
Top Choice & {\tt{American\_Broadcasting\_Company}} \\
Correct Choice & {\tt{Australian\_Broadcasting\_Corporation}} \\
Context & {\tt{$\ldots$he told ABC$\ldots$}} \\
Earlier Sentence & {\tt{$\ldots$he told the Australian Broadcasting Corporation$\ldots$}} \\
Heuristic & Looking for candidate Wikipedia titles that also match the target string,
{\tt{ABC}}, in the document,\\
&we find that the longest such title
is {\tt{Australian Broadcasting Corporation}} --- that of the correct entity.
\end{tabular}\end{center}}

\noindent
Notice that the last method --- looking for matching Wikipedia titles in a document ---
works correctly for all three examples.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

